Branch-and-bound for biobjective mixed-integer linear programming

We present a generic branch-and-bound algorithm for finding all the Pareto solutions of a biobjective mixed-integer linear program. The main contributions are new algorithms for obtaining dual bounds at a node, for checking node fathoming, presolve and duality gap measurement. Our branch-and-bound is predominantly a decision space search method since the branching is performed on the decision variables, akin to single objective problems, although we also sometimes split gaps and branch in the objective space. The various algorithms are implemented using a data structure for storing Pareto sets. Computational experiments are carried out on literature instances and also on a new set of instances that we generate using the MIPLIB benchmark library for single objective problems. We also perform comparisons against the triangle splitting method from literature, which is an objective space search algorithm.

==> miplib2.tex <==
\renewcommand{\dagger}{\ast}

\subsection{MIPLIB Instances}\label{sec:MIPLIB}
\revision{
Due to the successful results we obtained using our BB procedure on instances from the literature, we designed our second set of tests to measure the performance of our algorithm on a more challenging set of instances. For this we utilized a set of single objective MILP instances available from the MIPLIB 2017 library \cite[p]{miplib2017pre}. We chose only instances that were feasible, mixed-integer, contained at most 1000 total decision variables, and were marked easy. For each instance, we generated two secondary objective functions as follows:

\begin{enumerate}
\item[(r)] For each $i\in \{1,\dots,m+n\}$ the coefficient $c^2_i$ is randomly generated using the uniform distribution over the closed interval $\left[-\left\vert\max_i c^1_i\right\vert, \left\vert\max_i c^1_i\right\vert\right]$.
\item[(n)] We set $c^2_i = -c^1_i$.
\end{enumerate}

After generation of these instances we did some preliminary testing and discarded instances for which: (i) the Pareto set was a singleton, or (ii) the second objective was unbounded, or (iii) the MILP associated with either $f_1$ or $f_2$ took over 8 hours to solve. In the end, 104 instances remained for final testing (2 each, originating from 52 single objective MILP instances).

A primary reason for generating this additional set of instances is the relative ease with which single objective MILPs were solved throughout the solution process, both during the execution of triangle splitting and our \bb{}, when using the previously considered test sets. As such, in our first analysis of these new instances we set a variety of node limits on single objective MILPs solved during our \bb{} (other than the two specified on line 4 of Algorithm \ref{alg7}, of course). By limiting the number of nodes processed during each single objective MILP solve, we hoped to increase the speed of the overall \bb{} procedure while still being able to exploit useful dual bound information at each node. For initial tests, we set node limits of 10, $10^2$, $10^3$, $10^4$, and $\infty$ and compared the overall solution time for \bb{} on all 104 instances, with a maximum execution time of 8 hours. Surprisingly, the best performing node limits were $10^4$ and $\infty$. Hence, we opted to leave the single objective MILP node limit off for the remainder of our analysis. We did note, however, that on some instances, single objective MILPs took significant time to solve even when relatively few nodes were explored in order to do so. Thus, we opted to solve each instance again, this time with an overall time limit imposed when solving each single objective MILP. For this test we utilized time limits of 15, 30, 45, 60, 300, 1800, and $\infty$ seconds. In this case, the limits that appeared to produce the best results were 30 and 300 seconds, with 300 seconds having a slight advantage. We therefore imposed a single objective MILP time limit of 300 seconds when conducting our final round of tests.
}
%We then opted to test the performance of the various preprocessing procedures we tested in Section \ref{preprocess_test}, each set to a maximum execution time of either 5, 10 or 30 minutes. We then calculated the duality gap percentages after exiting preprocessing. The results of this test are displayed in the performance profile found in Figure \ref{prof}. Here ``ev'' represents the implementation of \textsc{PreprocessingMethod1} in which $\rho$ is calculated as a function of instance size, ``w0'' indicates \textsc{PreprocessingMethod2} with $\rho$ set to zero, and ``hy0'' indicates the hybrid preprocessing procedure with $\rho$ set to zero. The numbers following each of these represent the limits on execution time. 
%
%\begin{figure}%[H]
%\centering
%\includegraphics[width=\textwidth]{MIPLIB_preprocessing_profile}
%\caption{Performance profile of duality gap percentage for preprocessing procedures on instances from MIPLIB.}
%\label{prof}
%\end{figure}
%
%Observe from Figure \ref{prof} that \textsc{PreprocessingMethod1} with an execution time of 30 minutes performed the best. Hence, we utilized this procedure for our final test. In this test we used our original BB procedure, the BB procedure in which we exploit $\OS$ gaps, and the triangle splitting method on each of the instances generated from MIPLIB. We set a maximum time limit of 12 hours for each procedure. Additionally, we set a time limit of 60 seconds for all single objective MILPs solved during the course of our BB procedures, except for: (i) solving the initial MILPs associated with $f_1$ and $f_2$, and (ii) solving the MILPs necessary to appropriately reduce subregions of $\OS$ when employing our $\OS$ splitting procedure. We also note that we do not keep track of a duality gap measurement during the course of BB because doing causes a significant reduction in performance, especially when there are a large number of open nodes. Instead, we calculate this gap after termination of BB, but we only allow an additional 12 hours for this task. The results of this experiment are provided in detail in Table \ref{table_results}. and summarized by the performance profile in Figure \ref{MIPLIB_perf_prof}. Note that when constructing this profile we only included data for instances which were solved by at least one of the three methods for solving BOMILP. Hence, the maximum height of each curve is bounded by the fraction of instances solved in under twelve hours by at least one of the solution procedures.

% \begin{table}[H]
%%\tiny
%\centering
%%\footnotesize
%\caption{Experiment 8 -- Comparing with the triangle splitting method for instance from MIPLIB.}\label{table_results}
%\begin{tabular}{l|l|rrr|rrrr|r}
%\toprule
% &  & \multicolumn{3}{c}{Original BB}  & \multicolumn{4}{c}{BB with Gap Splitting} %& \multicolumn{3}{c}{Solved by one - St. dev.} 
% & \multicolumn{1}{c}{ T.S.} 	\\ 
%\cmidrule(r){3-5}
%\cmidrule(r){6-9}
%\cmidrule(r){10-10}
%Instance &  & Time & Nodes & $\overline{\mathcal{G}_{s^*}}$ & Time & $\dagger$ & Nodes & $\overline{\mathcal{G}_{s^*}}$& Time \\
%\midrule
%aflow40b          & o   & --    & 901   & *  & 2,181  & 2,181  & 2    & --  & 28,552 \\
%                  & a   & --    & 1,577 & *  & --     & --     & 1,658& --  & --\\
%		          & d    & 2,230 & 1     & -- & 12,099 & 12,095 & 166  & --  & 7,234 \\
%		          & e   & --    & 1,943  & *  & --     & --     & 1,259& *   & -- \\
%beasleyC3         & o   & --    & --    & -- & 751    & 749    & 3    & --  & -- \\
%                  & a   & --    & 888   & 14 & --     & --     & 9,076& 18  & -- \\
%                  & b   & --    & 697   & 24 & --     & --     & 533  & 100 & -- \\
%                  & e   & --    & 6,466 & *  & --     & --     &12,250& 13  & -- \\
%%berlin\_5\_8\_0 & 1 & 0 & 0 & 0 & -- 	  & --  & -- 	& -- & -- \\
%bienst2           & o & 1,596 & 35    & -- & 1,012  & 1,011 & 8     & --   & 2,174 \\
%binkar10\_1       & o & --    & 4,586 & *  & --     & --    & 5,461 & *    & -- \\
%                  & a & 3,229 & 921   & -- & 3,129  & 3,129 & 938   & --   & -- \\
%                  & b & 7,634 & 4,812 & -- & 7,555  & 7,555 & 4,433 & --   & 5,949 \\
%                  & c & 5,527 & 2,065 & -- & 8,587  & 3,238 & 8,587 & --   & -- \\
%                  & d & 6,892 & 1,313 & -- &  363   & 362   & 2     & --   & 2,360 \\
%                  & e & 4,684 & 286   & -- & 5,393  & 2,867 & 522   & --   & 25,293 \\
%csched007         & o & --    & 564   & 31 & --     & --    & 596   & 31   & -- \\
%                  & c & --    & 2,347 & 2  & --     & --    & 2,631 & 2    & -- \\
%csched010         & o & --    & 488   & 35 & --     & --    & 395   & 33   & --\\
%                  & a & --    & 515   & 16 & --     & --    & 683   & 16   & --\\
%                  & c & --    & 1,044 & 2  & 15,205 & 15,205& 1     & --   & --\\
%                  & d & --    & 589   & 100& 4,803  & 4,803 & 9     & --   & 32,811\\
%danoint           & o & 42,299& 538   & -- & 7,091  & 7,086 & 6     & --   & 41,880\\
%dfn-gwin-UUM      & o & --    & 859   & 67 & --     & --    & 1,953 & 100  & 25,434 \\
%gmu-35-40         & o & --    & 1,527 & 68 & --     & --    & 5,759 & 69   & 25,714\\
%                  & a & 2,072 & 1     & -- & --     & --    & 2,220 & 44   & --\\
%                  & d & --    & 559   & 2  & --     & --    & 719   & 4    & 9,973\\
%                  & e & 2,148 & 1     & -- & --     & --    & 2,715 & 44   & --\\
%gmu-35-50         & o & 2,804 & 1     & -- & 10,218 & 7,715 & 1,489 & --   & --\\
%                  & a & --    & 1,234 & 36 & --     & --    & 1,085 & 49   & --\\
%                  & e & --    & 907   & 41 & --     & --    & --    & --   & --\\
%ic97\_potential   & o & --    & 391   & 71 & --     & --    & 446   & 72   & --\\
%                  & a & --    & --    & -- & --     & --    & 17,248& 1    & 23,911\\
%                  & b & --    & 547   & 70 & --     & --    & 1,386 & 99   & --\\
%                  & d & --    & 297   & 97 & --     & --    & 340   & 93   & --\\
%k16x240           & o & --    & 17,648& 2  & --     & --    & 14,740& 2    & --\\
%                  & a & --    & 42,960& 6  & --     & --    & 23,837& *    & --\\
%                  & b & --    & 1,022 & 32 & --     & --    &187,846& 86   & --\\
%                  & c & --    & 2,418 & *  & --     & --    & 2,479 & *    & --\\
%                  & d & --    & 2,264 & *  & --     & --    & 3,542 & *    & --\\
%                  & e & --    & 17,251& 8  & --     & --    & 19,401& --   & --\\
%\bottomrule
%\multicolumn{8}{l}{\scriptsize $\dagger$ -- Approximated parallel time}\\
%\multicolumn{8}{l}{\scriptsize* -- duality gap calculation exceeded 12 hours} 
%\end{tabular}
%\end{table}
%
%%\renewcommand{\thetable}{\arabic{table} (Continued)}  
%%\addtocounter{table}{-1}
%
% \begin{table}[H]
%%\tiny
%\centering
%%\footnotesize
%\caption{(Continuation of Table \ref{table_results}.)}\label{table_results2}
%\begin{tabular}{l|l|rrr|rrrr|r}
%\toprule
% &  & \multicolumn{3}{c}{Original BB}  & \multicolumn{4}{c}{BB with Gap Splitting} %& \multicolumn{3}{c}{Solved by one - St. dev.} 
% & \multicolumn{1}{c}{ T.S.} 	\\ 
%\cmidrule(r){3-5}
%\cmidrule(r){6-9}
%\cmidrule(r){10-10}
%Instance &  & Time & Nodes & $\overline{\mathcal{G}_{s^*}}$ & Time & $\dagger$ & Nodes & $\overline{\mathcal{G}_{s^*}}$& Time \\
%\midrule
%%gmu-35-50         & o & 2,804 & 1     & -- & 10,218 & 7,715 & 1,489 & --   & --\\
%%                  & a & --    & 1,234 & 36 & --     & --    & 1,085 & 49   & --\\
%%                  & e & --    & 907   & 41 & --     & --    & --    & --   & --\\
%%ic97\_potential   & o & --    & 391   & 71 & --     & --    & 446   & 72   & --\\
%%                  & a & --    & --    & -- & --     & --    & 17,248& 1    & 23,911\\
%%                  & b & --    & 547   & 70 & --     & --    & 1,386 & 99   & --\\
%%                  & d & --    & 297   & 97 & --     & --    & 340   & 93   & --\\
%%k16x240           & o & --    & 17,648& 2  & --     & --    & 14,740& 2    & --\\
%%                  & a & --    & 42,960& 6  & --     & --    & 23,837& *    & --\\
%%                  & b & --    & 1,022 & 32 & --     & --    &187,846& 86   & --\\
%%                  & c & --    & 2,418 & *  & --     & --    & 2,479 & *    & --\\
%%                  & d & --    & 2,264 & *  & --     & --    & 3,542 & *    & --\\
%%                  & e & --    & 17,251& 8  & --     & --    & 19,401& --   & --\\
%markshare\_5\_0   & o & --    & 3,905 & 20 & --     & --    & 4,173 & 13   & 32,476\\
%                  & c & --    &117,984& 2  & --     & --    &166,057& 2    & 14,270\\
%                  & d & --    & 3,937 & 15 & 5,002  & 5,002 & 5     & --   & --\\
%mc11              & o & --    & 620   & 77 & --     & --    & 539   & *    & --\\
%                  & a & --    & 950   & *  & --     & --    & 6,071 & 13   & --\\
%                  & c & --    & 760   & 36 & --     & --    & 275   & *    & --\\
%                  & e & --    & 2,041 & *  & --     & --    & 918   & *    & --\\
%mcsched           & a & --    &14,578 & *  & --     & --    & 29,378& 20   & --\\
%                  & c & --    &14,040 & 0  & --     & --    & 19,954& 3    & --\\
%                  & d & --    & --    & -- & --     & --    & 9,588 & 0    & --\\
%mik-250-1-100-1   & o & --    & 9,882 & 6  & 404    & 404   & 3     & --   & --\\
%                  & a & --    & 17,814& 12 & --     & --    & 21,299& 64   & --\\
%                  & c & --    & 14,170& 0  & --     & --    & 14,217& *    & 32,204\\
%                  & d & --    & 11,972& *  & --     & --    & 8,889 & *    & --\\
%                  & e & --    & 1,434 & 21 & --     & --    & 1,116 & 59   & --\\
%neos-1112787      & a & 1,931 & 0     & -- & 1,891  & 1,890 & 3     & --   & -- \\
%                  & c & --    & 1,881 & *  & --     & --    & 1,681 & *    & -- \\
%neos-1171737      & o & 2,112 & 1     & -- & 2,210  & 2,210 & 1     & --   & --\\
%                  & d & --    & 677   & 33 & --     & --    & 673   & 81   & --\\
%neos-1225589      & b & --    & 410   & *  & --     & --    & 486   & *    & -- \\
%                  & c & --    & 1,260 & *  & --     & --    & 1,291 & *    & -- \\
%                  & d & --    & 16,214& *  & --     & --    & 44,389& --   & -- \\
%neos13            & o & --    & 1,779 & 16 & --     & --    & 3,466 & 100  & 12,383\\ 
%                  & a & --    & 488   & *  & --     & --    & 464   & *    & 25,263\\
%                  & c & 496   & 10    & -- & 574    & 559   & 11    & --   & 1,054\\  
%                  & d & --    & 12,625& 36 & --     & --    & 170   & 28   & --\\ 
%neos-1396125      & a & 824   & 50    & -- & 825    & 825   & 534   & --   & 535\\
%                  & b & 5,648 & 53    & -- & 3,713  & 3,590 & 28    & --   & 3,480\\
%                  & d & --    & 613   & *  & 2,111  & 2,103 & 4     & --   & 22,695\\
%neos-1426635      & d & --    & 2,761 & 30 & 1,203  & 1,203 & 2     & --   & 15,155\\
%neos-1426662      & d & 3,689 & 1     & -- & --     & --    & 651   & 27   & --\\
%neos-1440460      & d & --    & 999   & 35 & 1,903  & 1,903 & 1     & --   & --\\
%neos-1442657      & d & --    & 576   & 15 & 13,097 & 13,097& 1     & --   & --\\
%neos15            & a & --    & 15,811& 34 & --     & --    & 18,583& 34   & --\\
%                  & b & --    & 2,911 & *  & --     & --    & 2,911 & 42   & --\\
%neos-693347       & o & --    & 221   & *  & --     & --    & 2,670 & 56   & 11,480\\ 
%                  & c & 674   & 1     & -- & 673    & 673   & 1     & --   & 566\\ 
%                  & d & 722   & 1     & -- & 718    & 718   & 1     & --   & 566\\ 
%neos-916792       & o & --    & 757   & 51 & --     & --    & 794   & 49   & 3,662\\
%                  & a & 985   & 1     & -- & --     & --    & 5,257 & 0    & 426\\
%                  & c & --    & 3,874 & 2  & --     & --    & 3,465 & 11   & 6,657\\
%                  & d & --    & 672   & 70 & --     & --    & 666   & 79   & --\\
%neos-942830       & o & --    & 1,655 & 31 & --     & --    & 5,606 & 64   & --\\
%                  & a & 8,690 & 321   & -- & 9,952  & 9,952 & 271   & --   & 5,858\\
%                  & c & 3,711 & 1     & -- & 3,980  & 3,980 & 1     & --   & 5,344\\
%                  & d & 4,359 & 3     & -- & 3,057  & 3,057 & 3     & --   & --\\
%noswot            & o & 7,491 & 30,903& -- & 736    & 732   & 3,141 & --   & 1,069\\ 
%                  & a & --    & --    & -- & 754    & 753   & 10    & --   & --\\
%                  & c & 32,355& 5,699 & -- & --     & --    &254,933& 54   & 42,748\\
%                  & d & 1,942 & 1,092 & -- & 713    & 712   & 6     & --   & 878\\
%ns1830653         & o & 23,349& 665   & -- & 19,053 & 19,053& 458   & --   & 25,302\\
%                  & a & 19,242& 210   & -- & 18,110 & 18,110& 195   & --   & 10,363\\
%p80x400b          & o & --    & 7,024 & 6  & --     & --    & 7,778 & 6    & -- \\
%                  & a & --    & 16,439& 15 & --     & --    & 21,374& 17   & -- \\
%                  & b & --    & 641   & 58 & --     & --    & 62,581& 70   & -- \\
%                  & c & --    & 881   & *  & --     & --    & 2,205 & 0    & -- \\
%                  & d & --    & 1,589 & *  & --     & --    & 2,505 & 9    & -- \\
%                  & e & --    & 6,803 & 17 & --     & --    & 4,306 & 24   & -- \\
%pigeon-10         & o & 1,940 & 562   & -- & 1,656  & 1,656 & 1     & --   & 1,670 \\
%pigeon-11         & o & 20,436& 30    & -- & 20,266 & 20,266& 11    & --   & 20,672 \\
%qiu               & o & 1,665 & 326   & -- & 1,445  & 1,445 & 280   & --   & 4,100\\
%                  & a & 2,726 & 2,367 & -- & 1,911  & 873   & 686   & --   & 1,274\\
%                  & b & 19,706& 2,969 & -- & 1,888  & 1,886 & 5     & --   & 5,853\\
%                  & c & --    & 956   & 43 & 1,885  & 1,864 & 5     & --   & 4,146\\
%                  & d & --    & 41,745& 3  & 1,815  & 1,815 & 3     & --   & --\\
%                  & e & 4,809 & 541   & -- & 5,642  & 5,523 & 4,284 & --   & 834\\
%\bottomrule
%\multicolumn{8}{l}{\scriptsize $\dagger$ -- Approximated parallel time}\\
%\multicolumn{8}{l}{\scriptsize* -- duality gap calculation exceeded 12 hours}  
%\end{tabular}
%\end{table}
%
% \begin{table}[H]
%%\tiny
%\centering
%%\footnotesize
%\caption{(Second continuation of Table \ref{table_results}.)}\label{table_results3}
%\begin{tabular}{l|l|rrr|rrrr|r}
%\toprule
% &  & \multicolumn{3}{c}{Original BB}  & \multicolumn{4}{c}{BB with Gap Splitting} %& \multicolumn{3}{c}{Solved by one - St. dev.} 
% & \multicolumn{1}{c}{ T.S.} 	\\ 
%\cmidrule(r){3-5}
%\cmidrule(r){6-9}
%\cmidrule(r){10-10}
%Instance &  & Time & Nodes & $\overline{\mathcal{G}_{s^*}}$ & Time & $\dagger$ & Nodes & $\overline{\mathcal{G}_{s^*}}$& Time \\
%\midrule
%%neos-1396125      & a & 824   & 50    & -- & 825    & 825   & 534   & --   & 535\\
%%                  & b & 5,648 & 53    & -- & 3,713  & 3,590 & 28    & --   & 3,480\\
%%                  & d & --    & 613   & *  & 2,111  & 2,103 & 4     & --   & 22,695\\
%%neos-1426635      & d & --    & 2,761 & 30 & 1,203  & 1,203 & 2     & --   & 15,155\\
%%neos-1426662      & d & 3,689 & 1     & -- & --     & --    & 651   & 27   & --\\
%%neos-1440460      & d & --    & 999   & 35 & 1,903  & 1,903 & 1     & --   & --\\
%%neos-1442657      & d & --    & 576   & 15 & 13,097 & 13,097& 1     & --   & --\\
%%neos15            & a & --    & 15,811& 34 & --     & --    & 18,583& 34   & --\\
%%                  & b & --    & 2,911 & *  & --     & --    & 2,911 & 42   & --\\
%%neos-693347       & o & --    & 221   & *  & --     & --    & 2,670 & 56   & 11,480\\ 
%%                  & c & 674   & 1     & -- & 673    & 673   & 1     & --   & 566\\ 
%%                  & d & 722   & 1     & -- & 718    & 718   & 1     & --   & 566\\ 
%%neos-916792       & o & --    & 757   & 51 & --     & --    & 794   & 49   & 3,662\\
%%                  & a & 985   & 1     & -- & --     & --    & 5,257 & 0    & 426\\
%%                  & c & --    & 3,874 & 2  & --     & --    & 3,465 & 11   & 6,657\\
%%                  & d & --    & 672   & 70 & --     & --    & 666   & 79   & --\\
%%neos-942830       & o & --    & 1,655 & 31 & --     & --    & 5,606 & 64   & --\\
%%                  & a & 8,690 & 321   & -- & 9,952  & 9,952 & 271   & --   & 5,858\\
%%                  & c & 3,711 & 1     & -- & 3,980  & 3,980 & 1     & --   & 5,344\\
%%                  & d & 4,359 & 3     & -- & 3,057  & 3,057 & 3     & --   & --\\
%%noswot            & o & 7,491 & 30,903& -- & 736    & 732   & 3,141 & --   & 1,069\\ 
%%                  & a & --    & --    & -- & 754    & 753   & 10    & --   & --\\
%%                  & c & 32,355& 5,699 & -- & --     & --    &254,933& 54   & 42,748\\
%%                  & d & 1,942 & 1,092 & -- & 713    & 712   & 6     & --   & 878\\
%%ns1830653         & o & 23,349& 665   & -- & 19,053 & 19,053& 458   & --   & 25,302\\
%%                  & a & 19,242& 210   & -- & 18,110 & 18,110& 195   & --   & 10,363\\
%%p80x400b          & o & --    & 7,024 & 6  & --     & --    & 7,778 & 6    & -- \\
%%                  & a & --    & 16,439& 15 & --     & --    & 21,374& 17   & -- \\
%%                  & b & --    & 641   & 58 & --     & --    & 62,581& 70   & -- \\
%%                  & c & --    & 881   & *  & --     & --    & 2,205 & 0    & -- \\
%%                  & d & --    & 1,589 & *  & --     & --    & 2,505 & 9    & -- \\
%%                  & e & --    & 6,803 & 17 & --     & --    & 4,306 & 24   & -- \\
%%pigeon-10         & o & 1,940 & 562   & -- & 1,656  & 1,656 & 1     & --   & 1,670 \\
%%pigeon-11         & o & 20,436& 30    & -- & 20,266 & 20,266& 11    & --   & 20,672 \\
%%qiu               & o & 1,665 & 326   & -- & 1,445  & 1,445 & 280   & --   & 4,100\\
%%                  & a & 2,726 & 2,367 & -- & 1,911  & 873   & 686   & --   & 1,274\\
%%                  & b & 19,706& 2,969 & -- & 1,888  & 1,886 & 5     & --   & 5,853\\
%%                  & c & --    & 956   & 43 & 1,885  & 1,864 & 5     & --   & 4,146\\
%%                  & d & --    & 41,745& 3  & 1,815  & 1,815 & 3     & --   & --\\
%%                  & e & 4,809 & 541   & -- & 5,642  & 5,523 & 4,284 & --   & 834\\
%ran14x18          & o & --    & 2,610 & 8  & --     & --    & 4,424 & 8    & -- \\
%                  & a & --    & 40,881& 11 & --     & --    & 56,981& 12   & -- \\
%                  & b & --    & 875   & 33 & 3,074  & 3,073 & 4     & --   & -- \\
%                  & e & --    & 46,951& 14 & --     & --    & 40,132& 12   & 38,624 \\
%ran14x18-disj-8   & o & --    & 6,826 & 10 & --     & --    & 9,769 & 8    & -- \\
%                  & a & --    & 45,528& 27 & --     & --    & 68,137& 28   & 26,029 \\
%                  & b & --    & 922   & 30 & --     & --    & 648   & 1    & -- \\
%                  & e & --    & 10,727& 9  & --     & --    & 15,977& 11   & -- \\
%ran16x16          & o & --    & 12,180& 6  & --     & --    & 12,175& 6    & -- \\
%                  & a & --    & 23,189& *  & --     & --    & 25,738& *    & -- \\
%                  & e & --    & 19,916& 11 & --     & --    & 9,477 & *    & -- \\
%timtab1           & o & --    & 1,136 & 50 & --     & --    & 1,167 & 100  & -- \\
%                  & a & --    & 513   & 100& --     & --    & 535   & 100  & -- \\
%                  & b & --    & 575   & 100& --     & --    & 477   & 100  & -- \\
%                  & d & --    & 789   & 63 & --     & --    & 798   & 48   & -- \\
%%ran14x18          & o & --    & 2,610 & 8  & --     & --    & 4,424 & 8    & -- \\
%%                  & a & --    & 40,881& 11 & --     & --    & 56,981& 12   & -- \\
%%                  & b & --    & 875   & 33 & 3,074  & 3,073 & 4     & --   & -- \\
%%                  & e & --    & 46,951& 14 & --     & --    & 40,132& 12   & 38,624 \\
%%ran14x18-disj-8   & o & --    & 6,826 & 10 & --     & --    & 9,769 & 8    & -- \\
%%                  & a & --    & 45,528& 27 & --     & --    & 68,137& 28   & 26,029 \\
%%                  & b & --    & 922   & 30 & --     & --    & 648   & 1    & -- \\
%%                  & e & --    & 10,727& 9  & --     & --    & 15,977& 11   & -- \\
%%ran16x16          & o & --    & 12,180& 6  & --     & --    & 12,175& 6    & -- \\
%%                  & a & --    & 23,189& *  & --     & --    & 25,738& *    & -- \\
%%                  & e & --    & 19,916& 11 & --     & --    & 9,477 & *    & -- \\
%%timtab1           & o & --    & 1,136 & 50 & --     & --    & 1,167 & 100  & -- \\
%%                  & a & --    & 513   & 100& --     & --    & 535   & 100  & -- \\
%%                  & b & --    & 575   & 100& --     & --    & 477   & 100  & -- \\
%%                  & d & --    & 789   & 63 & --     & --    & 798   & 48   & -- \\
%\bottomrule
%\multicolumn{8}{l}{\scriptsize $\dagger$ -- Approximated parallel time}\\
%\multicolumn{8}{l}{\scriptsize* -- duality gap calculation exceeded 12 hours}  
%\end{tabular}
%\end{table}
%
%% \begin{table}[H]
%%%\tiny
%%\centering
%%%\footnotesize
%%\caption{(Third continuation of Table \ref{table_results}.)}\label{table_results4}
%%\begin{tabular}{l|l|rrr|rrrr|r}
%%\toprule
%% &  & \multicolumn{3}{c}{Original BB}  & \multicolumn{4}{c}{BB with Gap Splitting} %& \multicolumn{3}{c}{Solved by one - St. dev.} 
%% & \multicolumn{1}{c}{ T.S.} 	\\ 
%%\cmidrule(r){3-5}
%%\cmidrule(r){6-9}
%%\cmidrule(r){10-10}
%%Instance &  & Time & Nodes & $\overline{\mathcal{G}_{s^*}}$ & Time & $\dagger$ & Nodes & $\overline{\mathcal{G}_{s^*}}$& Time \\
%%\midrule
%%%neos-1396125      & a & 824   & 50    & -- & 825    & 825   & 534   & --   & 535\\
%%%                  & b & 5,648 & 53    & -- & 3,713  & 3,590 & 28    & --   & 3,480\\
%%%                  & d & --    & 613   & *  & 2,111  & 2,103 & 4     & --   & 22,695\\
%%%neos-1426635      & d & --    & 2,761 & 30 & 1,203  & 1,203 & 2     & --   & 15,155\\
%%%neos-1426662      & d & 3,689 & 1     & -- & --     & --    & 651   & 27   & --\\
%%%neos-1440460      & d & --    & 999   & 35 & 1,903  & 1,903 & 1     & --   & --\\
%%%neos-1442657      & d & --    & 576   & 15 & 13,097 & 13,097& 1     & --   & --\\
%%%neos15            & a & --    & 15,811& 34 & --     & --    & 18,583& 34   & --\\
%%%                  & b & --    & 2,911 & *  & --     & --    & 2,911 & 42   & --\\
%%%neos-693347       & o & --    & --    & -- & --     & --    & 2,670 & 56   & --\\ 
%%%                  & c & 674   & 1     & -- & 673    & 673   & 1     & --   & 566\\ 
%%%                  & d & 722   & 1     & -- & 718    & 718   & 1     & --   & 566\\ 
%%%neos-916792       & o & --    & 757   & 51 & --     & --    & 794   & 49   & 3,662\\
%%%                  & a & 985   & 1     & -- & --     & --    & 5,257 & 0    & 426\\
%%%                  & c & --    & 3,874 & 2  & --     & --    & 3,465 & 11   & 6,657\\
%%%                  & d & --    & 672   & 70 & --     & --    & 666   & 79   & --\\
%%%neos-942830       & o & --    & 1,655 & 31 & --     & --    & 5,606 & 64   & --\\
%%%                  & a & 8,690 & 321   & -- & 9,952  & 9,952 & 271   & --   & 5,858\\
%%%                  & c & 3,711 & 1     & -- & 3,980  & 3,980 & 1     & --   & 5,344\\
%%%                  & d & 4,359 & 3     & -- & 3,057  & 3,057 & 3     & --   & --\\
%%%noswot            & o & 7,491 & 30,903& -- & 736    & 732   & 3,141 & --   & 1,069\\ 
%%%                  & a & --    & --    & -- & 754    & 753   & 10    & --   & --\\
%%%                  & c & 32,355& 5,699 & -- & --     & --    &254,933& 54   & 42,748\\
%%%                  & d & 1,942 & 1,092 & -- & 713    & 712   & 6     & --   & 878\\
%%%ns1830653         & o & 23,349& 665   & -- & 19,053 & 19,053& 458   & --   & 25,302\\
%%%                  & a & 19,242& 210   & -- & 18,110 & 18,110& 195   & --   & 10,363\\
%%%p80x400b          & o & --    & 7,024 & 6  & --     & --    & 7,778 & 6    & -- \\
%%%                  & a & --    & 16,439& 15 & --     & --    & 21,374& 17   & -- \\
%%%                  & b & --    & 641   & 58 & --     & --    & 62,581& 70   & -- \\
%%%                  & c & --    & 881   & *  & --     & --    & 2,205 & 0    & -- \\
%%%                  & d & --    & 1,589 & *  & --     & --    & 2,505 & 9    & -- \\
%%%                  & e & --    & 6,803 & 17 & --     & --    & 4,306 & 24   & -- \\
%%%pigeon-10         & o & 1,940 & 562   & -- & 1,656  & 1,656 & 1     & --   & 1,670 \\
%%%pigeon-11         & o & 20,436& 30    & -- & 20,266 & 20,266& 11    & --   & 20,672 \\
%%%qiu               & o & 1,665 & 326   & -- & 1,445  & 1,445 & 280   & --   & 4,100\\
%%%                  & a & 2,726 & 2,367 & -- & 1,911  & 873   & 686   & --   & 1,274\\
%%%                  & b & 19,706& 2,969 & -- & 1,888  & 1,886 & 5     & --   & 5,853\\
%%%                  & c & --    & 956   & 43 & 1,885  & 1,864 & 5     & --   & 4,146\\
%%%                  & d & --    & 41,745& 3  & 1,815  & 1,815 & 3     & --   & --\\
%%%                  & e & 4,809 & 541   & -- & 5,642  & 5,523 & 4,284 & --   & 834\\
%%%ran14x18          & o & --    & 2,610 & 8  & --     & --    & 4,424 & 8    & -- \\
%%%                  & a & --    & 40,881& 11 & --     & --    & 56,981& 12   & -- \\
%%%                  & b & --    & 875   & 33 & 3,074  & 3,073 & 4     & --   & -- \\
%%%                  & e & --    & 46,951& 14 & --     & --    & 40,132& 12   & 38,624 \\
%%%ran14x18-disj-8   & o & --    & 6,826 & 10 & --     & --    & 9,769 & 8    & -- \\
%%%                  & a & --    & 45,528& 27 & --     & --    & 68,137& 28   & 26,029 \\
%%%                  & b & --    & 922   & 30 & --     & --    & 648   & 1    & -- \\
%%%                  & e & --    & 10,727& 9  & --     & --    & 15,977& 11   & -- \\
%%%ran16x16          & o & --    & 12,180& 6  & --     & --    & 12,175& 6    & -- \\
%%%                  & a & --    & 23,189& *  & --     & --    & 25,738& *    & -- \\
%%%                  & e & --    & 19,916& 11 & --     & --    & 9,477 & *    & -- \\
%%%timtab1           & o & --    & 1,136 & 50 & --     & --    & 1,167 & 100  & -- \\
%%%                  & a & --    & 513   & 100& --     & --    & 535   & 100  & -- \\
%%%                  & b & --    & 575   & 100& --     & --    & 477   & 100  & -- \\
%%%                  & d & --    & 789   & 63 & --     & --    & 798   & 48   & -- \\
%%\bottomrule
%%\multicolumn{8}{l}{\scriptsize $\dagger$ -- Approximated parallel time}\\
%%\multicolumn{8}{l}{\scriptsize* -- duality gap calculation exceeded 12 hours}  
%%\end{tabular}
%%\end{table}
%
%%\renewcommand{\thetable}{\arabic{table}} 

\input{miplib_table}

\input{miplib_table_size_primal_bound}

\revision{
Table~\ref{table_results} gives the results of this experiment, where the two lines for each instance correspond to the (r) and (n) methods, respectively, for generating the second objective function. Of the 104 instances considered, 46 were solved in under 8 hours by the original \bb{} implementation, 44 by the $\OS$ splitting \bb{} variant, and 64 by the triangle splitting method. Additionally, there were 8 instances which were solved in under 8 hours by at least one version of \bb{}, but not by the triangle splitting method, and 23 instances solved in under 8 hours by the triangle splitting method, but not by a \bb{} procedure. When \bb{} failed to complete in 8 hours, we allowed an additional hour for the computation of $\bar{\mathcal{G}}_{s^*}$. This computation was sometimes unsuccessful due to the extreme number of open nodes present upon termination. When it was successful, it is reported in Table~\ref{table_results} using the \percentGap{} symbol, otherwise we display a $\dagger$ symbol. Table~\ref{table_size_prim} gives the number of nondominated solutions stored when our BB terminated either by solving to optimality or reached its time limit.

In all, the results display comparable performance between the BB approaches and the triangle splitting method, though for instances in which there was a relative difference in performance, it was generally large. These discrepancies in performance seem to stem from overall structure of the Pareto set in $\OS$. In particular, triangle splitting appears have superior performance on instances for which either: (i) the total number of Pareto solutions is small, or (ii) most Pareto solutions are supported,  particularly if all Pareto solutions lie along a single line segment in $\OS$. The latter of these two properties was observed on the second variant of the ``markshare\_5\_0'' instance, for example. Additionally, both of these properties were observed in the Pareto sets of the second variant of instances beginning with ``mik,'' for example. To aid in the visualization of this property, we include Figure \ref{pareto_sets2} which displays the Pareto set and boundary of $\L_0$ for the (n) variants of the ``markshare\_5\_0'' and ``mik\_25\_20\_75\_1'' instances. On the other hand, \bb{} appears to have superior performance on instances for which either: (i) the total number of Pareto solutions is large, or (ii) a relatively large percentage of Pareto solutions are unsupported. We also note that occasionally numerical issues caused early termination of \bb{} when solving instances for which all Pareto solutions fall on a single line segment in $\OS$. In particular, for some such instances, the cutting plane generated on line 21 of Algorithm \ref{alg1} fell along this line segment in $\OS$ when the root node was processed. Thus, CPLEX determined that the duality gap here was 0 and terminated \bb{} execution prematurely. This phenomenon was observed on the (n) variant of the ``markshare\_4\_0,'' ``Nexp-50-20-1-1,'' and ``r50x360'' instances. This is indicated in Table \ref{table_results} using the \errorone{} symbol. In addition, the implementation of \bb{} which exploits $\OS$ gaps failed due to numerical issues on a small number of instances. This is indicated in Table \ref{table_results} using the \errortwo{} symbol.
}

\begin{figure}[h!]
\begin{subfigure}[h]{.55\textwidth}
\centering
\includegraphics[width=.9\textwidth]{../Figures/mark5_cropped_w_legend}
\caption{Variant (n) of the ``markshare\_5\_0'' instance.}
\label{mark5_v2}
\end{subfigure}%
\begin{subfigure}[h]{.45\textwidth}
\centering
\includegraphics[width=1\textwidth]{../Figures/mik1_cropped}
\caption{Variant (n) of the ``mik\_25\_20\_75\_1'' instance.}
\label{mik1_v2}
\end{subfigure}
\caption{Pareto set and boundary of $\L_0$ for two instances from MIPlib 2017.}%randomly selected instances from \citep{belotti2012biobjective} and \citep{boland2015acriterion}.}
\label{pareto_sets2}
\end{figure}

%There are two situations in which this occurred: (i) when all Pareto solutions on a BOMILP instance lie on a single line segment in $\OS$, and (ii) when there are an extremely low number of Pareto points or line segments. The former case seems to happen far less frequently than the latter, but it should be noted that in this case numerical issues can cause BB to terminate before all Pareto solutions are found if a cutting plane is generated which lies on the same segment in $\OS$ on which all Pareto solutions lie.
%
%In order to test the impact of the 60 second time limit placed on solving single objective MILPs, we repeated this experiment an additional two times, once with this time limit changed to 30 seconds, and once with it changed to 300 seconds. The results are summarized by the performance profile in Figure \ref{MIPLIB_perf_prof}. Note that when constructing this profile we only included data for instances which were solved by at least one of the utilized methods for solving BOMILP. Hence, the maximum height of each curve is bounded by the fraction of instances solved in under twelve hours by at least one of the solution procedures.
%\begin{figure}[h!]
%\centering
%\includegraphics[width=0.97\textwidth]{MIPLIB_profile3}
%\caption{Performance profile of relative CPU time for MIPLIB instances.}
%\label{MIPLIB_perf_prof}
%\end{figure}
%As with the results in Tables \ref{table_results}--\ref{table_results3}, this profile also displays comparable performance between the BB approaches and the triangle splitting method. On average our BB implementation in which objective space gaps are exploited and single objective MILPs are processed for a maximum of 300 seconds performs the best, while, interestingly, our standard BB with a MILP processing time of 300 seconds seems to perform the worst. 

